ST-BERT: Cross-modal Language Model Pre-training For End-to-end Spoken Language Understanding

Language model pre-training has shown promising results in various downstream tasks. In this context, we introduce a cross-modal pre-trained language model, called Speech-Text BERT (ST-BERT), to tackle end-to-end spoken language understanding (E2E SLU) tasks. Taking phoneme posterior and subword-level text as an input, ST-BERT learns a contextualized cross-modal alignment via our two proposed pre-training tasks: Cross-modal Masked Language Modeling (CM-MLM) and Cross-modal Conditioned Language Modeling (CM-CLM). Experimental results on three benchmarks present that our approach is effective for various SLU datasets and shows a surprisingly marginal performance degradation even when 1% of the training data are available. Also, our method shows further SLU performance gain via domain-adaptive pre-training with domain-specific speech-text pair data.

==> Tabels/results_smartlights_snips_00.tex <==
\begin{table}[t]
\begin{center}
\caption{Results on SmartLights dataset}
\label{table:smartlights}
\scriptsize
\begin{tabular}{l r r r r}
\\ \toprule 
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Far} & \multicolumn{2}{c}{Close} \\
 & Valid Acc & Test Acc & Valid Acc & Test Acc  \\ 
\midrule 
Huang et al. \cite{huang2020learning} & - & 47.38\% & - & 67.99\% \\
\midrule 
\textbf{AcousticXLM (Ours)} & \textbf{67.05\%} & \textbf{62.43\%} & \textbf{87.39\%} & \textbf{84.31\%} \\
\hline
- CM-CLM & 64.97\% & 60.83\% & 83.52\% & 81.12\% \\
- CM-MLM & 61.79\% & 58.00\% & 84.39\% & 80.86\% \\
(= MLM on speech only) & & & & \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


\begin{table}[t]
\begin{center}
\caption{Results on SNIPS dataset}
\label{table:snips}
\small
\begin{tabular}{l r r}
\\ \toprule 
Model & Valid Acc & Test Acc \\ 
\midrule 
\textbf{\axlm~(Ours)} & 97.00\% & \textbf{95.95\%} \\
\hline
- CM-CLM & 96.38\% & 94.90\% \\
- text data & \textbf{97.38\%} & 95.38\% \\
(= MLM-on speech only) & & \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> deprecated/Tables/dataset_statistics_00.tex <==
\begin{table}[t]
\begin{center}
\caption{Dataset statistics.}
\label{table:dataset}
\small
\begin{tabular}{c|c||c|c|c|c}
\multicolumn{6}{c}{} \\ \toprule
\multicolumn{2}{c||}{} & \textbf{train} & \textbf{valid} & \textbf{test} & \textbf{intents} \\ 
\midrule
\multicolumn{2}{c||}{FSC} & 23,132 & 3,118 & 3,793 & 31  \\ \hline
\multirow{2}{*}{SmartLights} & close & \multicolumn{3}{c|}{1765} & 6 \\
& far & \multicolumn{3}{c|}{1765} & 6  \\ \hline
\multicolumn{2}{c||}{Snips} & \multicolumn{2}{c|}{13084} & 700 & 7 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> deprecated/Tables/results_fsc_00.tex <==
\begin{table}[t]
\begin{center}
\caption{Results on the FSC dataset. 
% $\dagger$ denotes the result with data augmentation. 
`Use Text' implies that the model explicitly uses text data of FSC in training.}
\label{table:fsc}
\small
\begin{tabular}{l c r r}
\\ \toprule 
Model & Use Text & Valid Acc & Test Acc \\ 
%\midrule
% ASR-NLU \cite{wang2020large} & \textit{?} & - & 90.11\% \\ 
\midrule 
Lugosch et al. \cite{lugosch2019speech} & x & - & 98.80\% \\
Wang et al.  \cite{wang2020large} (BERT)  & x & - & 98.95\% \\
Wang et al. \cite{wang2020large} (ERNIE)  & x & - & 99.02\% \\
Denisov and Vu \cite{denisov2020pretrained} & o & - & 95.54\% \\
% Palogiannidi et al. \cite{palogiannidi2020end} & x & - & 98.85\%$^\dagger$ \\
Cho et al. \cite{cho2020speech} & o & - & 98.98\% \\
Price \cite{price2020end} & x & 94.8\% & 99.3\% \\
\midrule
\textbf{\axlm (Ours)} & x & \textbf{95.77\%} & \textbf{99.50\%} \\
\hline
- CM-CLM & x & 95.46\% & 99.42\% \\
- text data & x  & 95.45\% & 99.39\% \\
% (= MLM on speech only) &   & & \\
\hline
+ DAPT & o & \textbf{95.91\%} & \textbf{99.59\%} \\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}


==> deprecated/Tables/results_fsc_02.tex <==
\begin{table}[t]
\begin{center}
\caption{Results on the FSC dataset. $\dagger$ denotes the result with data augmentation. `Use Text' implies that the model explicitly uses text data of FSC in training.}
\label{table:fsc}
\small
\begin{tabular}{l c r r}
\toprule 
Model & Use Text & Valid Acc & Test Acc \\ 
\midrule
ASR-NLU \cite{wang2020large} & & - & 90.11\% \\ 
\midrule 
Lugosch et al. \cite{lugosch2019speech} &   & - & 98.80\% \\
Wang et al.  \cite{wang2020large} (BERT)  &  & - & 98.95\% \\
Wang et al. \cite{wang2020large} (ERNIE)  &  & - & 99.02\% \\
Denisov et al. \cite{denisov2020pretrained} & & - & \textit{95.54\%} \\
Palogiannidi et al. \cite{palogiannidi2020end} & - & - & \textit{98.85\%$^\dagger$} \\
Cho et al. \cite{cho2020speech} & o & - & 98.98\% \\
Price et al. \cite{price2020end} &  & 94.8\% & 99.3\% \\
\midrule
\textbf{\axlm~(Ours)} & x & \textbf{95.77\%} & \textbf{99.50\%} \\
\hline
- CM-CLM & x & 95.46\% & 99.42\% \\
- CM-MLM & x  & 95.45\% & 99.39\% \\
(= MLM on speech only) &   & & \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> deprecated/Tables/results_fsc_data_shortage_00.tex <==

\begin{table}[t]
\begin{center}
\caption{Accuracies of \axlm~in the data shortage scenarios on the FSC dataset.}
\label{table:fsc_shortage}
\small
\begin{tabular}{l c r r}
\toprule 
\multicolumn{1}{r}{\textit{\textbf{Data Shortage \#1}}} &\multicolumn{3}{c}{\textit{\textbf{10\%} (10 random subsets)}} \\
\midrule 
Model & Use Text & Valid Acc & Test Acc \\ 
\midrule
Lugosch et al. \cite{lugosch2019speech} &  & - & 97.96\% \\
Cho et al. \cite{cho2020speech} & o & - & 98.12\% \\
\midrule
\textbf{\axlm~(Ours)} & x & \textbf{93.10\%} & \textbf{99.13\%} \\
\hline
- CM-CLM & x & 92.45\% & 99.09\% \\
- CM-MLM & x  & 91.97\% & 99.04\% \\
(= MLM on speech only) &   & & \\
\hline
+ FSC text domain adaptation & o & \textbf{93.70\%} & \textbf{99.25\%} \\
\bottomrule\\ 
\toprule
\multicolumn{1}{r}{\textit{\textbf{Data Shortage \#2}}} &\multicolumn{3}{c}{\textit{\textbf{1\%} (20 random subsets)}} \\
\midrule 
Model & Use Text & Valid Acc & Test Acc \\ 
\midrule
Lugosch et al. \cite{lugosch2019speech} &  & - & 82.78\% \\
Cho et al. \cite{cho2020speech} & o & - & 83.12\% \\
\midrule
\textbf{\axlm~(Ours)} & x & 95.37\% & 95.64\% \\
\hline
- CM-CLM & x & \textbf{96.65\%} & \textbf{96.51\%} \\
- CM-MLM & x  & 77.51\% & 89.81\% \\
(= MLM on speech only) &   & & \\
\hline
+ DAPT & o & 95.53\% & 95.83\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> deprecated/Tables/results_fsc_data_shortage_02.tex <==

\begin{table}[t]
\begin{center}
\caption{Accuracies of \axlm~in the data shortage scenarios on the FSC dataset.}
\label{table:fsc_shortage}
\small
\begin{tabular}{l c r r}
\toprule 
\multicolumn{1}{r}{\textit{\textbf{Data Shortage \#1}}} &\multicolumn{3}{c}{\textit{\textbf{10\%} (10 random subsets)}} \\
\midrule 
Model & Use Text & Valid Acc & Test Acc \\ 
\midrule
Lugosch et al. \cite{lugosch2019speech} &  & - & 97.96\% \\
Cho et al. \cite{cho2020speech} & o & - & 98.12\% \\
\midrule
\textbf{\axlm~(Ours)} & x & \textbf{93.10\%} & \textbf{99.13\%} \\
\hline
- CM-CLM & x & 92.45\% & 99.09\% \\
- text data & x  & 91.97\% & 99.04\% \\
(= MLM on speech only) &   & & \\
\bottomrule\\ 
\toprule
\multicolumn{1}{r}{\textit{\textbf{Data Shortage \#2}}} &\multicolumn{3}{c}{\textit{\textbf{1\%} (20 random subsets)}} \\
\midrule 
Model & Use Text & Valid Acc & Test Acc \\ 
\midrule
Lugosch et al. \cite{lugosch2019speech} &  & - & 82.78\% \\
Cho et al. \cite{cho2020speech} & o & - & 83.12\% \\
\midrule
\textbf{\axlm~(Ours)} & x & 95.37\% & 95.64\% \\
\hline
- cross-model translation & x & \textbf{96.65\%} & \textbf{96.51\%} \\
- cross-modal mlm training & x  & 77.51\% & 89.81\% \\
(= audio mlm training only) &   & & \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> deprecated/Tables/results_fsc_data_shortage_03.tex <==

\begin{table}[t]
\begin{center}
\caption{Test accuracies of \axlm~in the data shortage scenarios on the FSC dataset. In these scenarios, 10\% and 1\%  of training data is used each to train.}
\label{table:fsc_shortage}
\small
\begin{tabular}{p{3.8cm} c r r}
\\ \toprule
Model & Use Text & \multicolumn{1}{c}{10\%} & \multicolumn{1}{c}{1\%} \\ 
\midrule
Lugosch et al. \cite{lugosch2019speech} & x & 97.96\% & 82.78\% \\
Cho et al. \cite{cho2020speech} & o & 98.12\% & 83.12\% \\
\midrule
\textbf{\axlm~(Ours)} & x & \textbf{99.13\%} & 95.64\% \\
\hline
- CM-CLM & x & 99.09\% & \textbf{96.51\%} \\
- text data & x  & 99.04\% & 89.81\% \\
% (= MLM on speech only) &   & & \\
\hline
+ DAPT & o & \textbf{99.25\%} & 95.83\% \\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}

==> deprecated/Tables/results_text_domain_adaptation_02.tex <==
\begin{table}[t]
\begin{center}
\caption{Results of text domain adaptation on the FSC dataset. In this case, the text data of the FSC dataset is used for pre-training.}
\label{table:fsc_da}
\small
\begin{tabular}{l c r r}
\\ \toprule 
The Amount of Train Data & Use Text & Valid Acc & Test Acc \\ 
\midrule
100\% & o & 95.91\% & 99.59\% \\
10\% & o & 93.70\% & 99.25\% \\
1\% & o & 95.53\% & 99.83\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> deprecated/experiment_00.tex <==
\section{Experiment}

\input{Tabels/results_fsc_00}

\subsection{Dataset}
We mainly evaluate our \jw{\axlm} on the Fluent Speech Command (FSC) dataset \cite{lugosch2019speech}, one of the most famous dataset for the end-to-end SLU tasks. This dataset includes 23,132 training utterances of 77 speakers, 3,118 validation utterances of 10 speakers, and 3,793 test utterances of 10 speakers. It contains 31 unique intents.
% Each utterance is annotated with intent, which is composed of three slots: action, object, and location. For example, an utterance ``turn on the lights'' is labeled as an intent \{action: ``activate'', object: ``lights'', location: ``none''\}. In FSC dataset, 31 unique intents exist in total.

Additionally, our model is validated on the Snips and SmartLight datasets for intent classification tasks.
Snips dataset is an NLU benchmark, which consists of utterances and their corresponding intent-slot labels \cite{coucke2018snips}. The numbers of training and test data are 13,084 and 700 respectively, including 7 unique intents. Previous SLU studies used this dataset by synthesizing audio from text data, and we followed \jw{the same experimental protocol.} To compare our result with the result of Huang and Chen, we used Google text-to-speech (TTS) system as they did \cite{huang2020learning}, though it does not guarantee that our audio data and their are the same.

SmartLights dataset is the subset of the Snips dataset. We use this dataset for validating the performance of our model where the number of data is small. SmartLights dataset consists of 1,765 commands related to smart lights, including 6 unique intents \cite{saade2018spoken}. The dataset has two kinds of audio data where microphone setting is different, close field and far field. The latter setting is more challenging. We use two repeated trial of 5-cross validation for validating our results, as we found that the result of single split has a high variance in this dataset.

% \subsection{Experimental Details}
% 일단 여기에 ``- cross-model translation'', ``- cross-modal mlm training'', ``+ FSC text domain adaptation'' 에 대한 설명을 적기

\subsection{Implementation}

\subsection{Results}

\input{Tabels/results_fsc_data_shortage_00}

\input{Tabels/results_smartlights_snips_01}

Table \ref{table:fsc} shows the accuracies of \axlm and comparative models on the FSC dataset. We try not to compare the model with data augmentation, for a fair comparison. Various type of data augmentation can be used, and the performance of our model would increase with data augmentation. However, for the paper which report only the result with data augmentation, we denote the result with $\dagger$. 
We also distinguish the results of the case where FSC text dataset is used. 
Some comparative models need FSC text information for each ASR instance \cite{cho2020speech}. 
% for knowledge distillation from text
However, additional text label on downstream task implies additional cost of labeling, which original end-to-end SLU models do not have to pay. We denote the case of using FSC text data in `Use Text' column.
\axlm also exploit text information of FSC dataset by audio-text domain adaptation. We also report the performance increase in the table \ref{table:fsc} and \ref{table:fsc_shortage}. 
% 우리는 text가 도움이 되는 것을 보였지만, 그 효과의 경향성에는 다소간의 차이가 있다는 것을 볼 수 있었다. 

As another ablation study, we also evaluate our model where some cross-modal pretraining is missing. 
Table \ref{table:fsc}, \ref{table:fsc_shortage}, and \ref{table:smartlights_snips} include the result of the ablation study. The overall trend of the ablation studies shows that cross-modal pretraining helps model performance.


To validate the efficiency of our model, we test our model in data shortage scenario as previous works did \cite{lugosch2019speech,cho2020speech}.
Table \ref{table:fsc_shortage} shows our model performs robustly even when the amount of data is small. Our model makes competitive results even when 10\% of training dataset is available comparing to previous methods which uses 100\% of training set. Moreover, in the 1\% scenario, error rate with comparative model is less than a third of comparative models.
In the 1\% setting, the number of the validation set is larger than that of the training set. We stick this setting to compare with previous study. Though, it seems the model overfits on the validation set, it also shows that the model also performs reasonably in the test set.

We also do additional experiments on the SNIPS and SmartLights dataset in Table \ref{table:smartlights_snips} to show that our model is robust to other dataset. 
Though we compare the result of Huang and Chen \cite{huang2020learning} in the table and try to make the experimental setting similar, the setting is not exactly same. In SmartLights dataset, random cross-validation is used for each study, and it is not verified that the synthetic audio from Google TTS is the same. Nevertheless, we compare the result to show that our model is competitive.


==> deprecated/experiment_02.tex <==
\section{Experiment}

% \input{Tabels/dataset_statistics_00}
\subsection{Training Details}
\emph{\textbf{Pre-traning. }}
%\subsection{Pre-Training Details}
We pre-trained the acoustic model and \axlm{} on 960 hours of Librispeech \cite{panayotov2015librispeech}. We use publicly available speech and text alignment\footnote{https://zenodo.org/record/2619474\#.X413GEIzZds}  \cite{lugosch2019speech} which is obtained using Montreal Forced Aligner \cite{mcauliffe2017montreal}. For the text input, we use WordPiece tokenizer \cite{wu2016google} to split the text. 

We adopt a curriculum pre-training \cite{wang2020curriculum} for better generalization and fast convergence \cite{bengio2009curriculum}. \axlm{} pre-training starts with CM-MLM task, the easier task, for the one-third of entire training and after then one of CM-MLM, speech-to-text, and text-to-speech CM-CLM tasks is sampled with an equal probability for every iteration during the rest of pre-training. 

\mj{We initialize the model parameters from BERT-base} and use Adam \cite{kingma2014adam} optimizer with linear-decay learning rate schedule where a peak learning rate is 1$\times $e-4. We train the model for about 160K steps with a 512 size of mini-batch where the maximum input sequence length is set to 256. 

\medskip
\noindent\emph{\textbf{Fine-tuning. }}
We mainly evaluate our \axlm{} on the Fluent Speech Command (FSC) dataset \cite{lugosch2019speech}, one of the most widely used datasets for the E2E SLU tasks. 
This dataset includes 23,132 training utterances of 77 speakers, 3,118 validation utterances of 10 speakers, and 3,793 test utterances of 10 speakers. It contains 31 unique intents.
% Each utterance is annotated with intent, which is composed of three slots: action, object, and location. For example, an utterance ``turn on the lights'' is labeled as an intent \{action: ``activate'', object: ``lights'', location: ``none''\}. In the FSC dataset, 31 unique intents exist in total.

Additionally, our model is validated on the Snips and SmartLight datasets for intent classification tasks.
Snips dataset is an NLU benchmark, which consists of utterances and their corresponding intent-slot labels \cite{coucke2018snips}. 
The number of training is 13,084 and validation and test data have 700 utterances respectively with 7 unique intents. 
Previous SLU studies used this dataset by synthesizing audio from text data, and we followed the same experimental protocol. To compare our result with the result of Huang and Chen, we used Google text-to-speech (TTS) system same as in \cite{huang2020learning}, though it does not guarantee that \jw{our synthesized data are identical to their audio.}%our audio data and their audio data are the same.

SmartLights dataset \cite{saade2018spoken} is the subset of the Snips dataset. We use this dataset for validating the performance of our model when the number of data is small. 
SmartLights dataset consists of 1,660 commands related to smart light, including 6 unique intents. 
\mj{For each utterance,} the dataset has two audio types
where microphone setting is different, close field and far field. The latter setting is more challenging. We use two repeated trials of ten-fold cross-validation for validating our results, as we found that the result of a single split has a high variance in this dataset.

%\mj{During fine-tuning, we selected the maximum sequence length either 128 or 256 depending on the dataset with a batch size of 32.}

% \subsection{Experimental Details}
% 일단 여기에 ``- cross-model translation'', ``- cross-modal mlm training'', ``+ FSC text domain adaptation'' 에 대한 설명을 적기

\subsection{Results}

\input{Tabels/results_fsc_00}

% \subsubsection{Main Results on the FSC Dataset}
\emph{\textbf{FSC Dataset.~}}
Table \ref{table:fsc} shows the accuracies of \axlm~and comparative models on the FSC dataset. We try not to compare the model with data augmentation, for a fair comparison. %Various type of data augmentation can be used, and the performance of our model would increase with data augmentation. 
% However, for the paper which report only the result with data augmentation, we denote the result with $\dagger$. 
We also show the result of the ablation study in Table \ref{table:fsc}, \ref{table:fsc_shortage}, and \ref{table:smartlights_snips}, where some cross-modal pretraining is missing.
% The overall trend of the ablation studies shows that cross-modal pretraining helps model performance.

\medskip \noindent
% \subsubsection{Results on Data Shortage Scenario}
\emph{\textbf{Data Shortage Scenario.~}}
To validate the efficiency of our model, we test our model in data shortage scenario as previous works did \cite{lugosch2019speech,cho2020speech}.
Table \ref{table:fsc_shortage} shows our model performs robustly even when the amount of data is small. We evaluate our model for 10 and 20 trials of different subsets, in 10\% and 1\% experiment, respectively. 
% Our model makes competitive results even when 10\% of training dataset is available comparing to previous methods which uses 100\% of training set. Moreover, in the 1\% scenario, error rate with comparative model is less than a third of comparative models.
% In the 1\% setting, the number of the validation set is larger than that of the training set. We stuck this setting to compare with previous study. Though, it seems the model overfits on the validation set, it also shows that the model also performs reasonably in the test set.

\input{Tabels/results_fsc_data_shortage_03}
% \input{Tabels/results_text_domain_adaptation_02}

%\subsubsection{Results on  Domain-Adaptation Pre-training} \label{DA}

\medskip \noindent
\emph{\textbf{Domain-Adaptive Pre-training (DAPT).~}}
We also distinguish the results of the case where the FSC text dataset is used. 
Some comparative models need FSC text information for each ASR instance \cite{cho2020speech}, whereas \axlm~does not.
Additional text label on downstream task implies additional cost of labeling, which original end-to-end SLU models do not have to pay. We denote the case of using FSC text data in `Use Text' column.
\axlm~also can exploit text information of FSC dataset by audio-text domain adaptation. We also report consistent performance increase in Table \ref{table:fsc} and \ref{table:fsc_shortage}.
%\ref{table:fsc_da}. 


\input{Tabels/results_smartlights_snips_01}

% \subsubsection{Results on the Snips and SmartLights Dataset}

\medskip \noindent
\emph{\textbf{Snips and SmartLights Dataset.~}}
We also do additional experiments on the Snips and SmartLights dataset in Table \ref{table:smartlights_snips} to show that our model is robust to other dataset. 
Though we compare the result of Huang and Chen \cite{huang2020learning} in the table and try to make the experimental setting similar, the setting is not exactly same. In SmartLights dataset, ten-fold cross-validation is used for each study, and it is not verified that the synthetic audio from Google TTS is the same for Snips dataset. Nevertheless, we compare the result to show that our model is competitive.

